Unsupervised Feature Clustering Improves Contrastive Representation Learning for Medical Image Segmentation

Self-supervised instance discrimination is an effective contrastive pretext task to learn feature representations and address limited medical image annotations. The idea is to make features of transformed versions of the same images similar while forcing all other augmented images' representations to contrast. However, this instance-based contrastive learning leaves performance on the table by failing to maximize feature affinity between images with similar content while counter-productively pushing their representations apart. Recent improvements on this paradigm (e.g., leveraging multi-modal data, different images in longitudinal studies, spatial correspondences) either relied on additional views or made stringent assumptions about data properties, which can sacrifice generalizability and applicability. To address this challenge, we propose a new self-supervised contrastive learning method that uses unsupervised feature clustering to better select positive and negative image samples. More specifically, we produce pseudo-classes by hierarchically clustering features obtained by an auto-encoder in an unsupervised manner, and prevent destructive interference during contrastive learning by avoiding the selection of negatives from the same pseudo-class. Experiments on 2D skin dermoscopic image segmentation and 3D multi-class whole heart CT segmentation demonstrate that our method outperforms state-of-the-art self-supervised contrastive techniques on these tasks.

==> section2_relatedworks.tex <==
One track of related works to this paper is about how to tackle the problem of limited annotated data for medical image segmentation. 



\section{Related Works}

\subsection{Self-supervised Learning in Natural Scene Images}

Self-supervised learning \cite{liu2021selfgenerativeorcontrastive} covers a wide range of approaches with a unified goal of learning useful representations through proxy (i.e. pretext) tasks without the need for annotations. 
\textbf{Traditional pretext tasks} use exemplars \cite{Dosovitskiy2016DiscriminativeUFexemplar}, patch position prediction \cite{Doersch2015UnsupervisedVRrelativepatch}, jigsaw solving \cite{noroozi2016jigsaw}, or rotation prediction \cite{gidaris2018unsupervisedrot} to learn transferable features. 
Others use generative approaches like patch in-panting \cite{Pathak2016ContextEFinpaint}, image colorization \cite{zhang2016colorization}, or GANs \cite{Radford2016UnsupervisedRLgan} to capture relevant features through appearance awareness. 

Recently, \textbf{contrastive learning} \cite{jaiswal2020surveycontrastive}\cite{oord2018representation} has outperformed previous paradigms via a metric learning approach where latent-space embeddings of similar images are encouraged to be close while representations of dissimlar images are pushed apart. 
Specifically, non-parametric instance discrimination \cite{wu2018unsupervisednonparametric}\cite{chen2020simple}\cite{chen2020mocov2}\cite{tian2020contrastivemultiviewcmc} has been popularly adopted.
However, in the context of medical images, treating all other images as another class is incongruent to semantic similarities commonly found across images. 
Other methods propose to only use positives \cite{grill2020bootstrapbyol}\cite{chen2021exploringsimsiam} (i.e. two transformed versions of the same image), however, this introduces other disadvantages such as lack of semantic diversity from a single image.

Related to our work, many approaches have leveraged \textbf{clustering for representation learning}. 
DeepCluster \cite{caron2018deepcluster} assigns the entire dataset to clusters after a set amount of iterations and predicts those clusters directly. 
Adopting metric learning ideas, SwAV \cite{caron2020unsupervisedswav} and ProtoNCE \cite{li2020prototypical} use learnable prototypes to structure the embedding space. 
SwAV \cite{caron2020unsupervisedswav}, specifically, is a seminal work that introduces an online clustering approach with differentiable prototypes (i.e. views). 
To learn embeddings, similar images are constrained to the same prototype assignment while dissimilar images are encouraged to have different view assignments. 
However, by learning features \& clustering concurrently, SwAV is more sensitive to initial cluster assignments, which may be exacerbated by the more subtle inter-class visual differences found in medical images.
% Although this approach also uses clustering to influence embedding distances, the amount of clusters is discrete \& fixed (i.e. akin to k-means), which is suboptimal for medical tasks where the number of classes and anatomical concepts vary meaningfully even among same-modality images. 
Moreover, all these methods have the disadvantage of having to set k clusters a priori while the quality of representations is highly dependent on this hyperparameter. 
This is suboptimal for medical tasks where the number of classes and anatomical concepts vary meaningfully even among same-modality images.
% Moreover, all these methods all have the disadvantage of having to set k clusters a priori while the quality of representations is highly dependent on this hyperparameter. 
Additionally, these approaches were designed for learning global features from natural scene images which have much richer intra- and inter-class appearances. 
It is common for two medical structures or objects to have very similar appearances but completely different categorizations. 
% We note that \textbf{cluster-based approaches in natural scene images} have also been proposed for representation learning. 



Similar to our proposal, \cite{sharma2020clusteringface} uses clustering to select positive \& negative samples for a contrastive loss.
However, their method utilizes DrLIM \cite{hadsell2006dimensionalityred} which only works with two samples.
Recent works have shown the advantages of non-parametric losses \cite{wu2018unsupervisednonparametric} as well as multiple negatives \cite{kalantidis2020hardneg} for improved contrastive learning. 


\subsection{Self-supervised Learning in Medical Images}

Many traditional self-supervised works have been adapted from natural scene approaches to medical image tasks like solving jigsaw puzzles \cite{zhu2020rubikp}, reconstructing images \cite{zhou2021modelsgenesis}, and position prediction \cite{Bai2019SelfSupervisedLF}. 
Recently, multiple contrastive learning approaches in medical images have also been proposed \cite{chen2021momentum}\cite{zhou2021preservational}. 
However, they use instance discrimination which ignores cross-image semantic similarities.
% Some of the popular works in this domain \textbf{YO ADD ITEMS HERE} are infamously known to only make use of positives from the same image. 
% They limit themselves to using global contrasting features exclusively and either do not consider or make very little efforts to use  available spatial priors. 
To address this, some works \cite{azizi2021bigmedical} \cite{Sowrirajan2021MoCoPIMetadata} \cite{vu2021medaug} propose the use of patient metadata to select more diverse positives. 
Meanwhile, the 3D counterparts to these methods \cite{chaitanya2020contrastive} \cite{Zeng2021PositionalCL} make assumptions on anatomical similarities based on slice positions across volumes.
However, these approaches assume that either meta-information relevant to image semantics is available or images have accessible spatial correspondences. 
Our approach uses unsupervised feature clustering to extract appearance-based features which requires no additional external requirements about the data.


\subsection{Clustering}

Here, we briefly discuss different clustering approaches. 
Note that our objective is not to propose novel clustering techniques but to select an appropriate method for the task of medical image contrastive learning. 

Clustering algorithms generally fall under four clusters.
They either rely on centroids \cite{scholkopf1998nonlinear} \cite{ben2001support}, densities \cite{ankerst1999optics} \cite{comaniciu2002mean} \cite{ester1996density} \cite{kriegel2011density}, distributions\cite{rasmussen1999infinite}\cite{xu1998distribution}, or are hierarchical \cite{zhang1996birch} \cite{guha1998cure} \cite{guha2000rock} \cite{karypis1999chameleon}. 
We further discuss the advantages and disadvantages of each type in the context of our problem setting in Sec. \ref{sec:methods1}.
For a more exhaustive study on clustering, we refer readers to \cite{xu2015comprehensiveclusteringsurvey}.



% We classify those works into two groups.
% \textbf{Data augmentation} tries to enlarge the dataset with the synthesized image and labels.
% For example,\cite{bowles2018gan} demonstrated improved performance in brain segmentation tasks after introducing GAN derived data to training set.
% \cite{chaitanya2019semi} used GAN to model the image transformation and also leveraged unlabeled dataset for generating data. 
% \textbf{Semi-supervised learning} takes advantage of the unlabeled data for additional information during training. 
% Self-training \cite{bai2017semi} updated models parameters after being trained with labeled and unlabeled data alternatively.
% ~\cite{zhang2017deep, li2020shape} introduced an adversarial network to distinguish segmentation result between images with annotations and without annotations so that the segmentation network finally generated segmentation of the same quality for the unlabeled data.
% Most recently, TCSM\cite{li2020transformation} added a regularization loss to encourage the segmentation result of the same unlabeled data after different perturbations to be the same.

% \textbf{Contrastive learning} belongs to pretext task and it is originally employed to learn image features that boost the subsequent classification task under self-supervised setting. 
% \cite{chen2020simple} forced the embedding features of an image to be similiar with that of the image after several transformations and dissimilar to all other images in the mini-batch in latent space.
% \cite{he2020momentum} built an dynamic queue and a moving-averaged encoder to increase the negative pairs in the batch.
% In terms of medical image segmentation, as far as we are aware, there are few works employing contrastive learning, including\cite{chaitanya2020contrastive, li2020contrastive}. \cite{li2020contrastive} added the contrastive loss to the cross entropy loss for joint training and was not targeted for limited annotation problem. 
